A Latent Transformer for Disentangled Face Editing in Images and Videos

High quality facial image editing is a challenging problem in the movie post-production industry, requiring a high degree of control and identity preservation. Previous works that attempt to tackle this problem may suffer from the entanglement of facial attributes and the loss of the person's identity. Furthermore, many algorithms are limited to a certain task. To tackle these limitations, we propose to edit facial attributes via the latent space of a StyleGAN generator, by training a dedicated latent transformation network and incorporating explicit disentanglement and identity preservation terms in the loss function. We further introduce a pipeline to generalize our face editing to videos. Our model achieves a disentangled, controllable, and identity-preserving facial attribute editing, even in the challenging case of real (i.e., non-synthetic) images and videos. We conduct extensive experiments on image and video datasets and show that our model outperforms other state-of-the-art methods in visual quality and quantitative evaluation. Source codes are available at https://github.com/InterDigitalInc/latent-transformer.

==> 5_video.tex <==
\input{fig/comparison_video}

\subsection{Overview}


In this section, we present a pipeline which applies the the proposed image editing method to the case of videos. The encoding process ensures that the encoded latent codes of two consecutive frames are similar to each other. Therefore, we can reconstruct a face video using the frames projected to the latent space of StyleGAN, which provides the basics for the next manipulation step. Thanks to the stability of our proposed latent transformer, the manipulation does not affect the consistency between the latent codes and generates stable edits on the projected frames. %
An overview of our proposed pipeline is presented in Figure \ref{video_pipeline}. The pipeline consists of three steps: pre-processing, image editing and seamless cloning.


\noindent \textbf{Pre-processing.} In order to edit the video in the latent space of StyleGAN, we first extract face images from the frames, according to the StyleGAN setting. We crop and align each frame around the face, following the pre-processing step of FFHQ dataset \cite{karras2019style}, on which the StyleGAN is pretrained. For face alignment we detect landmarks independently on each frame using a state-of-the-art method \cite{bulat2017far}. To avoid jitter, we further process the landmarks using optical flow between two consecutive frames and a Gaussian filtering along the whole sequence. All frames are cropped and aligned to have eyes at the center and resized to $1024 \times 1024$.%

\noindent \textbf{Image editing.} In this step, we apply our manipulation method on the processed face images. Each frame is encoded to the latent space of StyleGAN using the pre-trained encoder \cite{richardson2020encoding}. The encoded latent codes are processed by the proposed latent transformer to realize the attribute editing. The manipulated latent codes are further decoded by StyleGAN to generate the manipulated face images.

\noindent \textbf{Seamless cloning.} We use Poisson image editing method \cite{perez2003poisson} to blend the modified faces with the original input frames. In order to blend only the face area, we use the segmentation mask obtained from the detected facial landmarks.



\subsection{Video editing}

We apply our manipulation method on real-world videos collected from FILMPAC library \cite{filmpac}. Figure \ref{video_compare} shows the results of facial attribute editing on videos obtained from our proposed pipeline. From each input frame, we crop and align a face image and encode it to the latent space of StyleGAN with a pre-trained encoder \cite{richardson2020encoding}.
The encoded latent code is processed by the latent transformer to vary the target attribute, then decoded to an output face image and blended with the input frame. As can be seen from the results, our proposed method succeeds in removing the facial hair or adding the makeup, without influencing the consistency between the frames. Nevertheless, we also observe that the proposed method has more difficulty handling extreme pose (side face), which may be due to the limitation of the generation capacity of the StyleGAN model. Please refer to the supplementary material for more results on videos.






==> 7_unused.tex <==



\subsection{Ablation study}
\input{fig/classfier_table}
\input{fig/ablation_net}

In this section we discuss the choice of network architectures. Previous works \cite{shen2019interpreting, harkonen2020ganspace} on latent space manipulation search semantic directions in the latent space and realize attribute editing with simple linear interpolations. Nevertheless, the latent space for a pre-trained image generative network may be not well disentangled so that the semantic boundary is not necessarily linear. Given the obtained semantic boundary, the appropriate transformation direction may be different according to the position of latent code.

\textbf{Choise of Latent Classifier.} To predict the attributes on the latent codes, we train the classifier $\ve{C}_l$ in the latent space. We train several multi-layer perceptrons on our prepared dataset as mentioned in section \ref{sec:implementation}. Table \ref{classifier_table} reports an quantitative evaluation on the different choices of layers in the classifier. \PH{Maybe this is useless to say, but I presume you have computed these measures on test set. That may explain that the performance decreases for 4 layer due to overfitting effect.}Recall means the true positive rate while specificity is also referred to as true negative rate. Precision measures the proportion of the true positive samples among all the positive samples, while accuracy indicates the proportion of all the correct classified samples. $F_1$ score is the harmonic mean of precision and recall. As can be observed from the table, the 3-layer perceptron performs slightly better than all the others.

\textbf{Choice of Latent Transformer.} Our proposed latent transformer is a simple affine transformation \PH{Once again, I'd refer to a one-layer network. BTW, is it followed by a non-linear activation? If yes, it's not affine}. To compare the capacity of different choices of network architecture, we run our proposed baseline with three different MLPs: 1-layer, 2-layer and only bias. As shown in Figure \ref{ablation_net}, the choices of layers in the latent transformer does not influence the manipulations. Compared to the choice of a simple bias, an affine transformation allows to learn automatically the magnitude of edits according to the position of the latent code \PH{To be discussed together..}.


==> fig/ablation_net.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.98\linewidth]{fig/evaluation/ablation.png}
\caption{Attribute change vs. magnitude of edits. Each point marker represents a magnitude of edit, of which the position $x$ indicates the successful manipulation rate on the target attribute and $y$ indicates the average identity preservation score.
}
\label{ablation_net}
\end{figure}

==> fig/classfier_table.tex <==
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{P{0.16\linewidth}P{0.16\linewidth}P{0.18\linewidth}P{0.16\linewidth}P{0.16\linewidth}P{0.16\linewidth}}
\toprule
Classifier & Recall & Specificity & Precision & Accuracy & $F_1$ score
\\
\midrule
1-layer & 0,647 & 0,942 & 0,748 & 0,904 & 0,693\\
2-layer & 0,655 & 0,943 & 0,753 & 0,907 & 0,701\\
\textbf{3-layer} & 0,655 & 0,943 & 0,754 & 0,908 & 0,701\\
4-layer & 0,610 & 0,943 & 0,739 & 0,903 & 0,668\\
\bottomrule
\end{tabular}
\caption{\textbf{Choice of classifier}.}
\label{classifier_table}
\end{table}


